The power of a single Haar random state: constructing and separating quantum pseudorandomness

In this work, we focus on the following question: what are the cryptographic implications of having access to an oracle that provides a single Haar random quantum state? We find that the study of such a model sheds light on several aspects of the notion of quantum pseudorandomness. Pseudorandom states (PRS) are a family of states for which it is hard to distinguish between polynomially many copies of either a state sampled uniformly from the family or a Haar random state. A weaker notion, called single-copy pseudorandom states (1PRS), satisfies this property with respect to a single copy. We obtain the following results: 1. First, we show, perhaps surprisingly, that 1PRS (as well as bit-commitments) exist relative to an oracle that provides a single Haar random state. 2. Second, we build on this result to show the existence of an isometry oracle relative to which 1PRS exist, but PRS do not. Taken together, our contributions yield one of the first black-box separations between central notions of quantum pseudorandomness, and introduce a new framework to study black-box separations between various inherently quantum primitives.

==> commitment.tex <==
\section{Commitments in the CHRS model}
\label{sec:commitment}
This section describes an unconditional bit commitment protocol in the \CHRS\ model, and follows very closely the approach of \cite{morimae2023unconditionally} to compile a $\oprs$ into a commitment.

We adopt the definition of bit commitment with common reference state from \cite{morimae2023unconditionally} with the slight modification that the reference state must be Haar random. We point out another subtlety about this definition in Remark \ref{remark:3} below.

\begin{definition}[Bit commitment in the \CHRS\ model]
\label{def:com-in-chrs-model}
A non-interactive bit commitment scheme in the \CHRS\ model is given by a tuple of QPT algorithms: 
$C$ (the sender) and $R$ (the receiver). Let $\{\ket{\psi_\mylambda}\}_{\mylambda \in \mathbb{N}}$ denote the family of common Haar random states. The scheme consists of the following two phases.
\begin{itemize}
    \item \textbf{Commit phase}: The sender $C$ takes polynomially many copies of $\ket{\psi_\mylambda}$ and a bit $b \in \braces{0,1}$ as the input, generates a quantum state on registers $\sfC$ and $\sfR$, and sends register $\sfC$ to the receiver $R$.
    \item \textbf{Reveal phase}: $C$ sends $b$ and register $\sfR$ to R. R takes polynomially many copies of $\ket{\psi_\mylambda}$ and $(b, \sfC, \sfR)$ as input, and outputs either $b$ or $\perp$.
\end{itemize}
\end{definition}

\begin{remark}
\label{remark:3}
Note that in the above definition (which follows the style of \cite{morimae2023unconditionally}), for a given security parameter $\mylambda$, parties only have access to copies of the Haar random state $\ket{\psi_\mylambda}$. In contrast, in the definition of CHRS model that we gave in \cref{sec:1prs_CHRS}, the entire family $\{\ket{\psi_\mylambda}\}_{\mylambda \in \mathbb{N}}$ is available to all parties (who can request polynomially many copies, in the security parameter $\mylambda$). This distinction is important when proving an oracle separation, like our \cref{thm:oracle-sep}, because there we want to argue about the existence of a primitive relative to a \emph{fixed} oracle (rather than an oracle that changes for each value of the security parameter). However, this distinction is not as important in this section, given that our $\oprs$ construction, and the resulting commitment scheme, does in fact use only the single state $\ket{\psi_{\mylambda}}$ when the security parameter is $\mylambda$. So, we elect to use the simpler \cref{def:com-in-chrs-model} in this section for simplicity.
\end{remark}


Next, we define the notions of hiding and sum-binding for a bit commitment in the \CHRS\ model, analogously to \cite{CKR16} and \cite{morimae2023unconditionally}. We consider \emph{statistical} hiding with \emph{bounded access} to the common Haar random state, and \emph{statistical} sum-binding against adversaries that have even \emph{unbounded access} to the state.

\begin{definition}[Polynomial-copy statistical hiding] 
\label{def:poly-copy-statistical-hiding}
    A quantum commitment scheme $(C, R)$ in the \CHRS\ model is said to be polynomial-copy statistically hiding if for any computationally unbounded uniform algorithm $\calA$ and for any polynomial $t=t(\mylambda)$, there exists a negligible function $\negl$ such that, for all $\mylambda$,
    \begin{equation*}
    \begin{aligned}
        \Big\lvert\Pr_{\ket{\psi_n}\gets \mu_n} \Big[&1 \gets \calA\parens{1^\mylambda, \ket{\psi_\mylambda}^{\otimes t}, \tr_{\sfR}[\sigma_{\sfC, \sfR}] }:\sigma_{\sfC, \sfR} \gets C_{\text{com}}(\ket{\psi_\mylambda}^{\otimes r}, 0)\Big] \\ &-\Pr_{\ket{\psi_n}\gets \mu_n} \bracks{ 1 \gets \calA\parens{1^\mylambda, \ket{\psi_\mylambda}^{\otimes t}, \tr_{\sfR}[\sigma_{\sfC, \sfR}] }:\sigma_{\sfC, \sfR} \gets C_{\text{com}}(\ket{\psi_\mylambda}^{\otimes r}, 1)}\Big\rvert \leq \negl(\mylambda)
    \end{aligned}
    \end{equation*}
where $C_{\text{com}}$ is the ``commit phase'' of the sender algorithm $C$, and  $r = r(n)$ is the number of copies of the common Haar random state used by $C_{\text{com}}$.
\end{definition}

\begin{definition}[Statistical sum-binding]\label{def:sum-binding} 
    A commitment scheme $(C, R)$ in the \CHRS\ model satisfies statistical sum-binding if the following holds. Let $C_0^*$ and $C_1^*$ be any computationally unbounded malicious committers that take an unbounded number of copies of $\ket{\psi_n}$ as input, and behave identically in the ``commit phase''. Let $p_b$ be the probability that $R$ accepts the revealed bit $b$ in an interaction with $C_b^*$. Then, there exists a negligible function $\negl$ such that, for all $n$,
    \begin{equation*}
        p_0 + p_1 \leq 1 + \negl(\mylambda).
    \end{equation*}
\end{definition}

Following the approach in \cite{morimae2023unconditionally}, we will show that our commitment scheme satisfies a stronger binding condition, called ``extractor-based binding'', first introduced in \cite{AQY22}.

\begin{definition}[Statistical extractor-based binding]
\label{def:stat-extractor-based-binding}
    A commitment scheme in the \CHRS\ model $(C, R)$ satisfies statistical extractor-based binding if there is a computationally unbounded algorithm $\calE = \braces{\calE_{\mylambda}}_{\mylambda \in \N}$, called the extractor, such that for any unbounded time malicious committer $C^*$, the experiments $\mathsf{Real}_\mylambda^{C^*}$ and $\mathsf{Ideal}_\mylambda^{C^*, \calE}$ are statistically indistinguishable, i.e.\ an unbounded-time distinguisher cannot distinguish the two with  non-negligible advantage, where the experiments $\mathsf{Real}_\mylambda^{C^*}$ and $\mathsf{Ideal}_\mylambda^{C^*, \calE}$ are defined as follows. Let $\{\ket{\psi_\mylambda}\}_{\mylambda \in \mathbb{N}}$ denote the family of common Haar random states.
    \begin{itemize}
    \item $\mathsf{Real}_\mylambda^{C^*}$: The malicious committer $C^*$ takes polynomially many copies of $\ket{\psi_\mylambda}$ as input, and interacts with the honest receiver $R$ in the commit and reveal phases. Let $b \in \braces{0,1,\perp}$ be the output of $R$ and $\tau_{C^*}$ be the final state of $C^*$. The experiment outputs the pair $(\tau_{C^*}, b)$.
    \item $\mathsf{Ideal}_\mylambda^{C^*, \calE}$: $C^*$ takes $\ket{\psi_\mylambda}$ as input and runs its commit phase to generate a commitment $\sigma_\sfC$ where $C^*$ may keep a state that is entangled with $\sigma_{\sfC}$. $\calE_\mylambda$ takes the register $\sfC$ as input, outputs an extracted bit $b^* \in \braces{0,1}$, and sends a post-execution state on $\sfC$ (which might be different from the original one) to R as a commitment. Then $C^*$ and $R$ run the reveal phase. Let $b$ be the output of $R$ and $\tau_{C^*}$ be the final state of $C^*$. If $b \notin \braces{\perp, b^*}$, then the experiment outputs a symbol $\texttt{fail}$ and otherwise outputs a tuple $(\tau_{C^*}, b)$.
    \end{itemize}
\end{definition}


Morimae, Nehoran, and Yamakawa show the following result:
\begin{lemma}[{\cite[Lemma 7.6]{morimae2023unconditionally}}]
    Statistical extractor-based binding implies statistical sum-binding.
\end{lemma}

Our commitment protocol in the CHRS model takes essentially the same form as that in \cite{morimae2023unconditionally}. Let $\{\ket{\phi_k}\}_k$ be an $\oprs$ in the CHRS model. Let $\sfR$ and $\sfC$ be registers of the same size as $\ket{\phi_k}$. Then, to commit to $0$, the sender prepares 
$$ \sum_k (\ket{k}\ket{0})_{\sfR} \ket{\phi_k}_{\sfC} \,.$$
To commit to $1$, the sender prepares
$$ \sum_x \ket{x}_{\sfR} \ket{x}_{\sfC} \,,$$
i.e.\ the maximally entangled state across $\sfR$ and $\sfC$.

Substituting our $\oprs$ from \cref{fig:full-1prs-protocol}, we get the following construction, where the base commitment is repeated in parallel, and the reveal phase is carried out by using SWAP tests.


\vspace{0.5cm}
\begin{figure}[htb]
\centering
\begin{mdframed}[userdefinedwidth=0.8\textwidth, align=center]
    \textbf{Commitment phase}: the sender takes as input a bit $b \in \braces{0,1}$. Let
    $$ \ket{\tpsi_0}_{\sfR, \sfC} = \sum_{a, b \in \braces{0,1}^{0.45\mylambda}} \ket{ab\Vert 0^{0.1\mylambda}}_\sfR X^aZ^b\ket{\psi_\mylambda}_\sfC \,,$$
    and let
    $$\ket{\tpsi_1}_{\sfR, \sfC} =  \sum_{x \in \{0,1\}^n} \ket{x}_{\sfR} \ket{x}_{\sfC} \,.$$ 
    The sender prepares $\ket{\tpsi_b}^{\otimes n}_{\sfC_1 \ldots \sfC_n, \sfR_1 \ldots \sfR_n}$, and sends registers $\sfC_1 \ldots \sfC_n$ to the receiver.
    
    \vspace{1mm}
    \textbf{Reveal phase}: The sender sends $b$ and registers $\sfR_1 \ldots \sfR_n$ to the receiver. The receiver prepares the state $\ket{\tpsi_b}^{\otimes n}_{\sfC'_1 \ldots \sfC'_n, \sfR'_1 \ldots \sfR'_n}$, and performs a SWAP test between registers $(\sfC_1 \ldots \sfC_n, \sfR_1 \ldots \sfR_n)$ and $(\sfC'_1 \ldots \sfC'_n, \sfR'_1 \ldots \sfR'_n)$, and accepts if and only if all of the SWAP tests output 1.
\end{mdframed}
\caption{Quantum bit commitment scheme in the \CHRS\ model}
\label{fig:commitment-protocol}
\end{figure}

    
\begin{theorem}\label{thm:commitment-security}
The protocol in \cref{fig:commitment-protocol} satisfies polynomial-copy statistical hiding (as in \cref{def:poly-copy-statistical-hiding}) and statistical extractor-based binding (as in \cref{def:stat-extractor-based-binding}).
\end{theorem}
\begin{remark}
Notice that, since a commitment scheme in the plain model cannot be both statistically binding and hiding \cite{LC97,May97}, we also cannot, in the \CHRS\ model, simultaneously achieve statistical binding and $t$-copy statistical hiding for $t$ exponentially large in $n$. This is because when $t$ is exponentially large, an unbounded adversary can learn the common Haar random state $\ket{\psi_n}$ entirely via tomography. Hence, in this case, $t$-copy statistical hiding is equivalent to statistical hiding in the plain model.
\end{remark}
\begin{proof}[Proof of \cref{thm:commitment-security}]
\textbf{Polynomial-copy statistical hiding}. The $\sfC$ registers of $\ket{\tpsi_0}$ and $\ket{\tpsi_1}$ are respectively in the state $\rho_0 = \tr_{\sfR} \ket{\tpsi_0}\bra{\tpsi_0} = \frac{1}{2^{0.9\mylambda}} \sum_{a,b} {X^a Z^b \ket{\psi_\mylambda}\bra{\psi_\mylambda}X^aZ^b}$ and $\rho_1 = \tr_{\sfR} \ket{\tpsi_1}\bra{\tpsi_1} =\frac{1}{2^\mylambda} \sum_x \ket{x}\bra{x}$. These two states are indistinguishable even to an adversary with a polynomial number of copies of $\ket{\psi_n}$. In fact, using \cref{thm:1prs}, we have that for any $t = \poly (\mylambda)$, there is negligible function $\negl$, such that for all $n$,
\begin{equation*}
    \norm{\rho_0^{\otimes \mylambda} \otimes \psi^{\otimes t} - \rho_1^{\otimes \mylambda} \otimes \psi^{\otimes t}} \leq \mylambda \norm{\rho_0\otimes \psi^{\otimes t} - \rho_1\otimes \psi^{\otimes t}} = \negl(\mylambda)
\end{equation*}

\noindent \textbf{Statistical extractor-based binding}.

\begin{figure}[!htb]
\centering
\begin{mdframed}[userdefinedwidth=0.8\textwidth, align=center]
$\mathsf{Real}_\mylambda^{C^*}$:
\begin{enumerate}
    \item $C^*$ takes polynomially many copies of $\ket{\psi_\mylambda}$ as input and generates a state $\ket{\phi_b}$ over registers $(\sfC, \sfR, \sfW)$ along with a bit $b \in \{0,1\}$ where $\sfW$ is the work register of $C^*$.
    \item $C^*$ sends $\sfC$ to $R$ in the commit phase.
    \item $C^*$ sends $(b, \sfR)$ to $R$ in the reveal phase.
    \item $R$ runs the verification in the reveal phase. That is, $R$ takes as input $\ket{\psi_\mylambda}^{\otimes \mylambda}_{\sfC'}$, and $(b, \sfC, \sfR)$ from $C^*$; it prepares an ancilla register $\sfV$ in the state $\ket{0\dots 0}_\sfV$, applies the projective measurement $(P_b, \I-P_b)$ on registers $(\sfC', \sfC, \sfR, \sfV)$.
    \item If $R$ rejects (i.e.\ $R$ obtains the outcome corresponding to $\I-P_b$), $b$ is replaced by $\perp$.
    \item The experiment outputs $(b, \sfW)$.
\end{enumerate}
$\mathsf{Ideal}^{C^*, \calE}$:
\begin{enumerate}
    \item $C^*$ takes polynomially many copies of $\ket{\psi_\mylambda}$ as input and generates a state $\ket{\phi_b}$ over registers $(\sfC, \sfR, \sfW)$ along with a bit $b \in \{0,1\}$ where $\sfW$ is the work register of $C^*$.
    \item $C^*$ sends $\sfC$ to $R$ in the commit phase.
    \item The extractor $\calE_\mylambda$ prepares the ancilla register $\sfE$ in the state $\ket{0\dots 0}_\sfE$, applies the projective measurement $\{\tilde{\Pi}_0,\tilde{\Pi}_1, \tilde{\Pi}_\perp\}$ on registers $\sfC$ and $\sfE$, and lets $b^* \in \{0,1,\perp\}$ be the outcome. $\calE_\mylambda$ sends $\sfC$ to $R$.
    \item $C^*$ sends $(b, \sfR)$ to $R$.
    \item $R$ runs the verification in the reveal phase. That is, $R$ takes as input $\ket{\psi_\mylambda}^{\otimes \mylambda}_{\sfC'}$, and $(b, \sfC, \sfR)$ from $C^*$; it prepares an ancilla register $\sfV$ in the state $\ket{0\dots 0}_\sfV$, applies the projective measurement $(P_b, \I-P_b)$ on registers $(\sfC', \sfC, \sfR, \sfV)$.
    \item If $R$ accepts (i.e.\ $R$ obtains the outcome corresponding to $P_b$) and $b \neq b^*$, the experiment outputs the special symbol $\mathsf{fail}$ and halts.
    \item If $R$ rejects (i.e.\ $R$ obtains the outcome corresponding to $\I-P_b$), $b$ is replaced by $\perp$.
    \item The experiment outputs $(b, \sfW)$.
\end{enumerate}
\end{mdframed}
\caption{$\mathsf{Real}_\mylambda^{C^*}$ and $\mathsf{Ideal}_\mylambda^{C^*, \calE}$}
\label{fig:extractor-binding}
\end{figure}

To show that the construction satisfies the statistical extractor-based binding property we need two technical lemmas.
\begin{lemma}[{\cite[Lemma 2] {harrow2013testing}}]
\label{lem:swap-test-fidelity}
    Let $m \in \mathbb{N}$. Let $\rho$ be a quantum state over $m$ registers $\sfA_1, \dots, \sfA_m$. Let $\sigma$ be a quantum state over $m$ registers $\sfB_1, \dots, \sfB_m$. Consider the following test, applied to $\rho \otimes \sigma$:
    \begin{enumerate}
        \item For each $i \in [m]$, do the SWAP test between $\sfA_i$ and $\sfB_i$.
        \item Accept if all SWAP tests are successful
    \end{enumerate}
    Then the success probability that the above test accepts is $\frac{1}{2^m}\sum_{S\subseteq [m]} \tr [\rho_S\sigma_S]$, where $\rho_{S}$ is the state obtained by tracing out all registers $\sfA_i$ of $\rho$ such that $i \notin S$, and $\sigma_S$ is the state obtained by tracing out all registers $\sfB_i$ of $\sigma$ such that $i \notin S$.
\end{lemma}

\begin{lemma}[{\cite[Lemma 31]{Yan22}}]\label{lem:proj-fidelity}
    Let $\ket{\tpsi_0}_{\sfX, \sfY}$ and $\ket{\tpsi_1}_{\sfX, \sfY}$ be pure states over registers $(\sfX, \sfY)$ such that
    \begin{equation*}
        F\left(\tr_\sfY[\ket{\tpsi_0}\bra{\tpsi_0}_{\sfX,\sfY}], \tr_\sfY[\ket{\tpsi_1}\bra{\tpsi_1}_{\sfX. \sfY}]\right) = \eps
    \end{equation*}
    Then there is a projective measurement $\{\Pi_0, \Pi_1, \Pi_\perp \coloneqq \I-\Pi_0-\Pi_1 \}$ over registers $\sfX$ such that for each $b \in \{0,1\}$,
    \begin{equation*}
        \norm{(\Pi_{b})_\sfX\otimes \I_{\sfY}\ket{\tpsi_b}_{\sfX, \sfY}}^2 \geq 1-\sqrt{2\eps}
    \end{equation*}
\end{lemma}

Recall that we defined the reduced state of the honest commitment states $\ket{\tpsi_0}_{\sfC\sfR}$ and $\ket{\tpsi_1}_{\sfC\sfR}$ on the $\sfC$ registers respectively as $\rho_0 = \tr_{\sfR} \ket{\tpsi_0}\bra{\tpsi_0} = \frac{1}{2^{0.9\mylambda}} \sum_{a,b} {X^a Z^b \ket{\psi_\mylambda}\bra{\psi_\mylambda}X^aZ^b}$ and $\rho_1 = \tr_{\sfR} [\ket{\tpsi_1}\bra{\tpsi_1}] =\frac{1}{2^\mylambda} \sum_x \ket{x}\bra{x}$.

Since the rank of $\rho_0$ does not exceed $2^{0.9\mylambda}$, while $\rho_1 = \frac{\mathds{1}}{2^\mylambda}$, it is straightforward to show that $\norm{\rho_0- \rho_1} \geq 1 - \frac{2^{0.9\mylambda}}{2^\mylambda} = 1-\negl(\mylambda)$ (by taking the eigendecomposition of $\rho_0$). Set $\epsilon = 1 - \norm{\rho_0-\rho_1} = \negl(\mylambda)$. According to \cref{lem:proj-fidelity}, there exists a family of orthogonal projectors $\braces{\Pi_0, \Pi_1, \Pi_{\perp} = \I - \Pi_0 - \Pi_1}$ on $\sfC$ such that for each $b \in \braces{0,1}$, it holds that
\begin{equation}\label{eq:proj-psib-bound}
    \norm{(\I-\Pi_b)_\sfC \otimes \I_\sfR \ket{\tpsi_b}}^2 \leq \sqrt{2\epsilon} \,.
\end{equation}

We define the extractor $\calE_\mylambda$ as follows:
\begin{itemize}
\item Upon receiving the commitment register $\sfC = (\sfC_1, \dots, \sfC_\mylambda)$, for each $i \in [\mylambda]$, apply the projective measurement $\braces{\Pi_0, \Pi_1, \Pi_\perp}$ on $\sfC_i$ to obtain an outcome $b_i \in \braces{0,1,\perp}$.
\item 
\begin{itemize}
    \item If $\abs{\braces{i \in [\mylambda]: b_i = 0}}>2\mylambda/3$, output $b^*=0$.
    \item If $\abs{\braces{i \in [\mylambda]: b_i = 1}}>2\mylambda/3$, output $b^*=1$.
    \item Otherwise, output $b^* = \perp$
\end{itemize}
\end{itemize}


We can equivalently describe $\calE_\mylambda$ as some projective measurement $\braces{\tilde{\Pi}_0, \tilde{\Pi}_1, \tilde{\Pi}_\perp}$ on register $\sfC$ and an ancilla register $\sfE$ initialized as $\ket{0\ldots 0}_\sfE$. 

For $b\in \braces{0,1}$, let $(P_b, \I-P_b)$ be the projective measurement corresponding to the ``purified'' verification performed by the receiver $R$ in the reveal phase. That is, $(P_b, \I-P_b)$ is defined so that $R$ is described as follows: on input $\ket{\psi_\mylambda}^{\otimes n}_{\sfC'}$, where $\sfC' \coloneqq \sfC'_1 \ldots \sfC'_n$, as well as $(b, \sfC, \sfR)$ from the sender, $R$ initializes an ancilla register $\sfV$ to $\ket{0\dots 0}_\sfV$, and applies the projective measurement $(P_b, \I-P_b)$ to all previous registers. $R$ accepts if the outcome is the former, and rejects if its the latter. 

Let $C^*$ be a malicious sender. Then, concretely, the experiments $\mathsf{Real}_\mylambda^{C^*}$ and $\mathsf{Ideal}_\mylambda^{C^*, \calE}$ are as in \cref{fig:extractor-binding}.

In what follows, for simplicity, we omit writing identities on registers were operators act trivially. Let $\ket{\phi_b}$ be defined as in \cref{fig:extractor-binding}. We define the mixed states $\rho_{\mathsf{real}}(b)$ and $\rho_{\mathsf{ideal}}(b)$ to correspond to the outputs of $\mathsf{Real}_\mylambda^{C*}$ and $\mathsf{Ideal}_\mylambda^{C^*, \calE}$ conditioned on the bit sent from $C^*$ being $b$. That is, we let\footnote{To see that these are the correct definitions one can use the ciclicity of the partial trace.}
\begin{equation}\label{eq:def-rho-real}
    \rho_{\mathsf{real}}(b) \coloneqq \tr_{\sfC', \sfC, \sfR, \sfV, \sfE}[P_b\ket{\tilde{\phi_b}}\bra{\tilde{\phi_b}}]\otimes \ket{b}\bra{b} + \tr_{\sfC', \sfC, \sfR, \sfV, \sfE}[(\I-P_b)\ket{\tilde{\phi_b}}\bra{\tilde{\phi_b}}]\otimes \ket{\perp}\bra{\perp}
\end{equation}
and
\begin{equation}\label{eq:def-rho-ideal}
   \begin{aligned}
    \rho_{\mathsf{ideal}}(b) \coloneqq& \tr_{\sfC', \sfC, \sfR, \sfV, \sfE}[N_b\ket{\tilde{\phi_b}}\bra{\tilde{\phi_b}}]\otimes \ket{b}\bra{b} + \tr_{\sfC', \sfC, \sfR, \sfV, \sfE}[N_\perp\ket{\tilde{\phi_b}}\bra{\tilde{\phi_b}}]\otimes \ket{\perp}\bra{\perp} \\& + \tr_{\sfC', \sfC, \sfR, \sfV, \sfE}[N_{\texttt{fail}}\ket{\tilde{\phi_b}}\bra{\tilde{\phi_b}}]\otimes \ket{\texttt{fail}}\bra{\texttt{fail}}
\end{aligned} 
\end{equation}

where
\begin{equation*}
   \ket{\tilde{\phi}_b} \coloneqq \ket{\phi_b}_{\sfC, \sfR, \sfW} \otimes \ket{\psi_{\mylambda}}_{\sfC'}^{\otimes \mylambda} \otimes \ket{0\dots 0}_\sfV \otimes \ket{0 \dots 0}_\sfE 
\end{equation*}
and
\begin{equation*}
N_b\coloneqq\tilde{\Pi}_bP_b\tilde{\Pi}_b,\, N_{\texttt{fail}} \coloneqq (\I-\tilde{\Pi}_b)P_b(\I-\tilde{\Pi}_b),\, N_\perp \coloneqq \I - N_b - N_{\texttt{fail}}.
\end{equation*}
Noting that the distribution of $b$ is identical in both experiments, it suffices to prove
\begin{equation*}
    \norm{\rho_{\mathsf{real}}(b) - \rho_{\mathsf{ideal}}(b)} = \negl(\mylambda)
\end{equation*}
for $b \in \braces{0,1}$. We show the following lemma. 
\begin{lemma}\label{lem:extractor-fail-bound}
    For each $b \in \braces{0, 1}$, it holds that
    \begin{equation*}
\norm{(P_b)_{\sfC,\sfR,\sfC',\sfV}(\I-\tilde{\Pi}_b)_{\sfC,\sfE}\ket{\tilde{\phi}_b}}^2 = \negl(\mylambda) \,.
    \end{equation*}
\end{lemma}
\begin{proof}

By definition of $P_b$ and $\ket{\tilde{\phi}_b}$, $\norm{P_b(\I-\tilde{\Pi}_b)\ket{\tilde{\phi}_b}}^2$ is the probability that the bit extracted from $\ket{\tilde{\phi}_b}$ is not $b$ \emph{and} the residual state passes the verification performed by $R$ with respect to $b$.
%the residual state $\rho \coloneqq \tr_{\sfW, \sfE} \parens{(I-\tilde{\Pi}_b)_{\sfC, \sfE} \ket{\phi_b}_{\sfC,\sfR,\sfW} \ket{0\dots 0}_{\sfE}}$ passes the verification performed by $R$ with respect to the committed bit $b$. 
Let $\rho_{\sfC, \sfR} \coloneqq \tr_{\sfW, \sfE} \left[(\I-\tilde{\Pi}_b)_{\sfC, \sfE} \ket{\phi_b}\bra{\phi_b}_{\sfC,\sfR,\sfW} \otimes \ket{0\dots 0}\bra{0\dots 0}_{\sfE}\right]$.
By \cref{lem:swap-test-fidelity}, this probability is equal to
    \begin{equation*}
        \frac{1}{2^\mylambda} \sum_{S\subseteq [n]}\tr [\rho_S\sigma_S]
    \end{equation*}
    where $\sigma \coloneqq \bigotimes_{i \in [\mylambda]} \ket{\tpsi_b}\bra{\tpsi_b}$. Here $\rho_S$ and $\sigma_S$ are the states obtained by tracing out all $\sfC_i \sfR_i$, respectively $\sfC'_i \sfR'_i$, for $i \notin S$. Notice that the latter expression for the probability takes into account the fact that $\rho$ is sub-normalized.
    
    By the definition of $\tilde{\Pi}_b$, we can write
    \begin{equation*}
        \rho = \sum_{T \subseteq [\mylambda], |T| \leq 2\mylambda/3} \tr_{\sfW} \left[{\hat{\Pi}_b^{(T)}} \ket{\phi_b} \bra{\phi_b} \hat{\Pi}_b^{(T)}\right]
    \end{equation*}
    where
    \begin{equation*}
        \hat{\Pi}_b^{(T)} = \parens{\bigotimes_{i\in T} (\Pi_b)_{\sfC_i}} \otimes \parens{\bigotimes_{i \notin T} (\I-\Pi_{b})_{\sfC_i}} \,.
    \end{equation*}
    We have
    \begin{align*}
        \frac{1}{2^\mylambda} &\sum_{S \subseteq [\mylambda]} \tr \left[\rho_S\sigma_S \right] \\&= \frac{1}{2^\mylambda} \sum_{S \subseteq [\mylambda]}\sum_{T\subseteq [\mylambda]:|T|\leq 2\mylambda/3} \tr \left[\parens{ \tr_{\braces{\sfC_i, \sfR_i}_{i \notin S},\sfW} \hat{\Pi}_b^{(T)} \ket{\phi_b} \bra{\phi_b} \hat{\Pi_b}^{(T)} } \parens{\bigotimes_{i \in S} \ket{\tpsi_b}\bra{\tpsi_b}_{\sfC_i, \sfR_i}} \right] \,.
    \end{align*}
    Now, for any $S$ and $T$, we have
    \begin{align*}
        &\tr \left[\parens{ \tr_{\braces{\sfC_i, \sfR_i}_{i \notin S},\sfW} \hat{\Pi}_b^{(T)} \ket{\phi_b} \bra{\phi_b} \hat{\Pi_b}^{(T)} } \parens{\bigotimes_{i \in S} \ket{\tpsi_b}\bra{\tpsi_b}_{\sfC_i, \sfR_i}}\right] \\
        =&\tr \left[\parens{ (\I-\Pi_b)^{\otimes|S\backslash T|}_{\braces{\sfC_i}_{i \in S\backslash T}} \parens{\tr_{\braces{\sfC_i, \sfR_i}_{i \notin S},\sfW} \hat{\Pi}_b^{(T)}  \ket{\phi_b} \bra{\phi_b} \hat{\Pi_b}^{(T)}}(\I-\Pi_b)^{\otimes|S\backslash T|}_{\braces{\sfC_i}_{i \in S\backslash T}} } \parens{\bigotimes_{i \in S} \ket{\tpsi_b}\bra{\tpsi_b}_{\sfC_i, \sfR_i}} \right] \\
        =& \tr \left[\parens{\tr_{\braces{\sfC_i, \sfR_i}_{i \notin S},\sfW} \hat{\Pi}_b^{(T)}  \ket{\phi_b} \bra{\phi_b} \hat{\Pi_b}^{(T)}}(\I-\Pi_b)^{\otimes|S\backslash T|}_{\braces{\sfC_i}_{i \in S\backslash T} } \parens{\bigotimes_{i \in S} \ket{\tpsi_b}\bra{\tpsi_b}_{\sfC_i, \sfR_i}}(\I-\Pi_b)^{\otimes|S\backslash T|}_{\braces{\sfC_i}_{i \in S\backslash T}} \right] \\
        \leq& \norm{\hat{\Pi}_b\ket{\phi_b}}^2 \tr \left[(\I-\Pi_b)^{\otimes|S\backslash T|}_{\braces{\sfC_i}_{i \in S\backslash T}} \parens{\bigotimes_{i \in S} \ket{\tpsi_b}\bra{\tpsi_b}_{\sfC_i, \sfR_i}}(\I-\Pi_b)^{\otimes|S\backslash T|}_{\braces{\sfC_i}_{i \in S\backslash T}} \right] \\
        \leq& \norm{\hat{\Pi}_b\ket{\phi_b}}^2 \norm{(\I-\Pi_b)\ket{\tpsi_b}}^{2|S\backslash T|} \\
        \leq& \norm{\hat{\Pi}_b\ket{\phi_b}}^2 (\sqrt{2\eps})^{|S\backslash T|} \,,
    \end{align*}
    where the final inequality follows from \cref{eq:proj-psib-bound}, where $\eps = \negl(n)$. 

    Thus for any $T$ such that $|T|\leq 2\mylambda/3$, we have
    \begin{align*}
        &\frac{1}{2^\mylambda} \sum_{S \subseteq [\mylambda]} \tr \left[\parens{ \tr_{\braces{\sfC_i, \sfR_i}_{i \notin S},\sfW} \hat{\Pi}_b^{(T)} \ket{\phi_b} \bra{\phi_b} \hat{\Pi_b}^{(T)} } \parens{\bigotimes_{i \in S} \ket{\tpsi_b}\bra{\tpsi_b}_{\sfC_i, \sfR_i}} \right]\\
        \leq &\,\,\frac{1}{2^\mylambda} \sum_{S\subseteq [\mylambda]}\norm{\hat{\Pi}_b^{(T)} \ket{\phi_b}}^2 (\sqrt{2\eps})^{|S\backslash T|}\\
        \leq &\,\,\norm{\hat{\Pi}_b^{(T)} \ket{\phi_b}}^2 \cdot \frac{1}{2^\mylambda} \parens{ \sum_{S \subseteq [\mylambda]: S \subseteq T} 1 + \sum_{S \subseteq [\mylambda]: S \not\subseteq T} \sqrt{2\eps}} \\
        \leq& \,\,\, 2^{-\mylambda/3}+\sqrt{2\eps} \,.
    \end{align*}
    where the final inequality follows directly from $|\braces{S \subseteq [\mylambda]: S \subseteq T}| = 2^{|T|} \leq 2^{2\mylambda/3}$.

    Therefore, we have
    \begin{equation*}
        \frac{1}{2^\mylambda} \sum_{S \subseteq [\mylambda]} \tr[\rho_S\sigma_S]
        \leq 2^{-\mylambda/3}+\sqrt{2\eps} \leq \negl(\mylambda) \,.
    \end{equation*}
\end{proof}

Recall the definitions of $\rho_{\mathsf{real}}(b)$ and $\rho_{\sf{ideal}}(b)$ from Equations \eqref{eq:def-rho-real} and \eqref{eq:def-rho-ideal} respectively. Let $\tau_{\sf{real}}^{(b)}$ and $\tau_{\sf{real}}^{(\perp)}$ be such that
\begin{equation*}
\rho_{\mathsf{real}}(b) = \tau_{\sf{real}}^{(b)} \otimes \ket{b}\bra{b} + \tau_{\sf{real}}^{(\perp)} \otimes \ket{\perp}\bra{\perp}\,,
\end{equation*}
and let $\tau_{\sf{ideal}}^{(b)}, \tau_{\sf{ideal}}^{(\perp)}, \tau_{\sf{ideal}}^{(\texttt{fail})}$ be such that
\begin{equation*}
\rho_{\sf{ideal}}(b) = \tau_{\sf{ideal}}^{(b)} \otimes \ket{b}\bra{b} + \tau_{\sf{ideal}}^{(\perp)} \otimes \ket{\perp}\bra{\perp} + \tau_{\sf{ideal}}^{(\texttt{fail})} \otimes \ket{\texttt{fail}}\bra{\texttt{fail}} \,.
\end{equation*}
We can now use \cref{lem:extractor-fail-bound} to show the following fact.
\begin{lemma}\label{lem:tau-trace-distance-bound}
    For each $b \in \braces{0,1}$, the following hold:
    \begin{enumerate}
        \item $\tr \left[\tau_{\sf{ideal}}^{(\texttt{fail})} \right] = \negl(\mylambda)$
        \item $\norm{\tau_{\sf{ideal}}^{(b)} - \tau_{\sf{real}}^{(b)}} = \negl(\mylambda)$
         \item $\norm{\tau_{\sf{ideal}}^{(\perp)} - \tau_{\sf{real}}^{(\perp)}} = \negl(\mylambda)$ \,.
    \end{enumerate}
\end{lemma}
\begin{proof}
    For the first item, we have
    \begin{equation*}
        \tr[\tau_{\sf{ideal}}^{(\texttt{fail})}] = \tr [N_{\sf{fail}}\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}] = \braket{\tilde{\phi}_b | (\I-\tilde{\Pi}_b)P_b(\I-\tilde{\Pi}_b)|\tilde{\phi}_b} = \norm{P_b(\I-\tilde{\Pi}_b)\ket{\tilde{\phi}_b}}^2 = \negl(\mylambda) \,,
    \end{equation*}
    where the last equality is by \cref{lem:extractor-fail-bound}.

    For the second item, we have 
    \begin{align*}
        \norm{\tau_{\sf{ideal}}^{(b)} - \tau_{\sf{real}}^{(b)}}&\leq \norm{P_b\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}P_b - P_b\tilde{\Pi}_b\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}\tilde{\Pi}_bP_b} \\
        &= 2\max_Q \tr \left[Q\parens{P_b\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}P_b - P_b\tilde{\Pi}_b\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}\tilde{\Pi}_bP_b}\right] \\
        &\quad - \left[\tr(P_b\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}P_b) - \tr(P_b\tilde{\Pi}_b\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}\tilde{\Pi}_bP_b)\right] \\
        &=2\max_Q \big(\norm{QP_b\ket{\tilde{\phi}_b}}^2 - \norm{QP_b\tilde{\Pi}_b\ket{\tilde{\phi}_b}}^2 \big) -  \big(\norm{P_b\ket{\tilde{\phi}_b}}^2 - \norm{P_b\tilde{\Pi}_b\ket{\tilde{\phi}_b}}^2 )
    \end{align*}
    where the maximum is taken over all projectors $Q$ on $(\sfW, \sfC', \sfC, \sfR, \sfV, \sfE)$, and the first inequality follows from the fact that trace distance is decreasing under taking a partial trace. For any projector $Q$, we have
    \begin{align*}
        \bigg| \big\|QP_b &\ket{\tilde{\phi}_b}\|^2 - \big\|QP_b\tilde{\Pi}_b\ket{\tilde{\phi}_b}\big\||^2 \bigg|\\
        =& \abs{\norm{QP_b(\tilde{\Pi}_b+(\I-\tilde{\Pi}_b)) \ket{\tilde{\phi}_b}}^2 - \norm{QP_b\tilde{\Pi}_b\ket{\tilde{\phi}_b}}^2} \\
        =& \abs{\braket{\tilde{\phi}_b|P_b Q P_b (\I-\tilde{\Pi}_b) |\tilde{\phi}_b} + \braket{\tilde{\phi}_b|(\I- \tilde{\Pi}_b) P_b Q P_b \tilde{\Pi}_b |\tilde{\phi}_b}}\\
        \leq & \,\,2 \norm{P_b(\I-\tilde{\Pi}_b)} = \negl(\mylambda) \,,
    \end{align*}
    where the last equality is by \cref{lem:extractor-fail-bound}.
    
    Finally, for the third item, we have
    \begin{align*}
        \norm{\tau_{\sf{real}}^{(\perp)} - \tau_{\sf{ideal}}^{(\perp)}} =& \norm{\tr_{\sfC', \sfC, \sfR, \sfV, \sfE} \left[(\I-P_b)\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b} \right] - \tr_{\sfC', \sfC, \sfR, \sfV, \sfE}\left[(\I-N_b-N_{\sf{fail}})\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}\right] } \\
        =& \norm{\tr_{\sfC', \sfC, \sfR, \sfV, \sfE}\left[(N_b+N_{\sf{fail}}-P_b)\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b} \right]  } \\
        \leq& \norm{\tr_{\sfC', \sfC, \sfR, \sfV, \sfE}\left[(N_b-P_b)\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b}\right]} + \tr \left[(N_{\sf{fail}}\ket{\tilde{\phi}_b}\bra{\tilde{\phi}_b} \right]= \negl(\mylambda) \,,
    \end{align*}
    where the last line follows from the triangle inequality, as well as the first and second item.
\end{proof}
We can now bound the distance between $\rho_{\sf{real}}(b)$ and $\rho_{\sf{ideal}}(b)$ as
\begin{equation*}
    \norm{\rho_{\sf{real}}(b) - \rho_{\sf{ideal}}(b)} = \norm{\tau_{\sf{real}}^{(b)} - \tau_{\sf{ideal}}^{(b)}} + \norm{\tau_{\sf{real}}^{(\perp)} - \tau_{\sf{ideal}}^{(\perp)}} +  \tr \left[\tau_{\sf{ideal}}^{(\texttt{fail})} \right] = \negl(\mylambda)
\end{equation*}
where the last equality follows from \cref{lem:tau-trace-distance-bound}. This yields the desired statistical binding property, and completes the proof of \cref{thm:commitment-security}.
\end{proof}

==> errata.tex <==
\subsection{Lifting the PRS attack to the unitary model}
In this section, we will show how to lift the $\prs$ attack in the CHRS model to the unitary model. The issue here is that given a $\prs$ in the unitary model, we can simulate a global-phase twirling of the $\prs$ in the CHRS model. But in fact, the global-phase twirling is enough for the $\prs$ attack, as shown later in this section.

The attack in the unitary model is a slight modification of the attack in~\cref{sec:oracle-sep}. Let us recall the attack in~\cref{sec:oracle-sep} first. Let $\gen_k$ be the generation unitary of the $\prs$ when the secret key is $k$. The adversary can take copies of $\ket{\psi}$ and apply $\gen_k$ on it. Then the adversary applies (multiple copies of) the swap test $\{\Pi_{sym}, I-\Pi_{sym}\}$ on it. 

But in the unitary model, the generation algorithm $\gen_k$ makes queries to the unitary oracle $U_{\ket{\psi}}$. According to~\cref{thm:isometry-to-unitary}, given polynomial many copies of $\ket{\psi}$, there is an efficient unitary $\widetilde{\gen}$ that applies on copies of $\ket{\psi}$ and outputs a state close to the global-phase twirled $\prs$ $\E_{\alpha} \gen^{U_{\alpha\ket{\psi}}}\ket{0}\bra{0}\gen^{U_{\alpha\ket{\psi}}, \dagger}$, denoted as $\rho_k$. The good news here is that $\rho_{k,\psi}$ has an inverse polynomial overlap with  $\gen_k\ket{0}$.

\begin{lemma}\label{lem:state-simulation-overlap}
    Assume that $\gen_k$ makes at most $T$ queries to $U_{\psi}$, then with exception probability at most $\exp(-O(N/T^2))$, $\braket{0|\gen_k^{\dagger}|\rho_{k,\psi}|\gen_k|0} \geq \frac{1}{3T}$.
\end{lemma}
\begin{proof}
    First, we will show the average of the overlap $\braket{0|\gen_k^{\dagger}|\rho_{k,\psi}|\gen_k|0}$ is at least $\frac{1}{2T+1}$. In fact,
    \begin{align*}
        \E_{\psi} \braket{0|\gen_k^{U_{\ket{\psi}},\dagger}|\rho_{k, \psi}|\gen_k^{\ket{\psi}}|0} &= \E_{\psi, \alpha} \braket{0|\gen_k^{U_{\alpha\ket{\psi}},\dagger}|\rho_{k,\psi}|\gen_k^{\alpha\ket{\psi}}|0} \\
        &= \E_{\psi} \tr \rho_{k, \psi}^2 \\
        &\geq \E_\psi \frac{1}{2T+1} = \frac{1}{2T+1},
    \end{align*}
    where the last inequality stems from the fact that $\rho_{k, \psi}$ is of rank at most $2T+1$ (Recall the proof in~\cref{sec:unitaryoracle1} that the counting register $\sfC$ ranges from $-T$ to $T$ so there are at most $2T+1$ branches in the purification of $\rho_{k, \psi}$) and Cauchy-Schwarz inequality.

    Thus according to~\cref{lem:levy-lemma}, except for probability at most $\exp(-O(N/T^2))$, the overlap $\braket{0|\gen_k^{\dagger}|\rho_{k,\psi}|\gen_k|0}$ is $O(1/T)$-close to the average (as a result, greater than $1/3T$).
\end{proof}

Now we can replace the projector $\Pi_k$ in~\cref{eq:projectors_attack} with
\begin{align*}
    \widetilde{\Pi_k} = \left(\Big((\widetilde{U_k}^\dagger)_{\mathsf{AB}} \otimes \I_{\mathsf{C}} \Big) (\Pi^{sym}_{\mathsf{AC}} \otimes \I_{\mathsf{B}} )\Big((\widetilde{U_k})_{\mathsf{AB}} \otimes \I_{\mathsf{C}}\Big)\right)^{\otimes \poly},
\end{align*}
where $\widetilde{U_k}$ is the unitary operator corresponding to $\widetilde{\gen}_k$. Then according to~\cref{lem:state-simulation-overlap}, $\ket{\phi_k}^{\otimes \poly} \otimes \ket{\psi}^{\otimes \poly}$ will pass the test with high probability, and $\ket{\phi}^{\otimes \poly} \otimes \ket{\psi}^{\otimes \poly}$ cannot pass the test with high probability, and then plug in the OR lemma~\cref{lem:or-lemma}, we are done. 

\begin{comment}
\subsection{Lifting the PRS attack to the unitary model}
In this section, we will show how to lift the $\prs$ attack in the CHRS model to the unitary model. The issue here is that given a $\prs$ in the unitary model, we can simulate a global-phase twirling of the $\prs$ in the CHRS model. But in fact, the global-phase twirling is enough for the $\prs$ attack, as shown later in this section.

The attack in the unitary model is a slight modification of the attack in~\cref{sec:oracle-sep}. Let us recall the attack in~\cref{sec:oracle-sep} first. Let $\gen_k$ be the generation unitary of the $\prs$ when the secret key is $k$. The adversary can take copies of $\ket{\psi}$ and apply $\gen_k$ on it. Then the adversary applies (multiple copies of) the swap test $\{\Pi_{sym}, I-\Pi_{sym}\}$ on it. 

But in the unitary model, the generation algorithm $\gen_k$ makes queries to the unitary oracle $U_{\ket{\psi}}$. According to~\cref{thm:isometry-to-unitary}, given polynomial many copies of $\ket{\psi}$, there is an efficient unitary $\widetilde{\gen}$ that applies on copies of $\ket{\psi}$ and outputs a state close to the global-phase twirled $\prs$ $\E_{\alpha} \gen^{U_{\alpha\ket{\psi}}}\ket{0}\bra{0}\gen^{U_{\alpha\ket{\psi}}, \dagger}$, denoted as $\rho_k$. The good news here is that $\rho_{k,\psi}$ has an inverse polynomial overlap with  $\gen_k\ket{0}$.

\begin{lemma}\label{lem:state-simulation-overlap}
    Assume that $\gen_k$ makes at most $T$ queries to $U_{\psi}$, then with exception probability at most $\exp(-O(N/T^2))$, $\braket{0|\gen_k^{\dagger}|\rho_{k,\psi}|\gen_k|0} \geq \frac{1}{3T}$.
\end{lemma}
\begin{proof}
    First, we will show the average of the overlap $\braket{0|\gen_k^{\dagger}|\rho_{k,\psi}|\gen_k|0}$ is at least $\frac{1}{2T+1}$. In fact,
    \begin{align*}
        \E_{\psi} \braket{0|\gen_k^{U_{\ket{\psi}},\dagger}|\rho_{k, \psi}|\gen_k^{\ket{\psi}}|0} &= \E_{\psi, \alpha} \braket{0|\gen_k^{U_{\alpha\ket{\psi}},\dagger}|\rho_{k,\psi}|\gen_k^{\alpha\ket{\psi}}|0} \\
        &= \E_{\psi} \tr \rho_{k, \psi}^2 \\
        &\geq \E_\psi \frac{1}{2T+1} = \frac{1}{2T+1},
    \end{align*}
    where the last inequality stems from the fact that $\rho_{k, \psi}$ is of rank at most $2T+1$ (Recall the proof in~\cref{sec:unitaryoracle1} that the counting register $\sfC$ ranges from $-T$ to $T$ so there are at most $2T+1$ branches in the purification of $\rho_{k, \psi}$) and Cauchy-Schwarz inequality.

    Thus according to~\cref{lem:levy-lemma}, except for probability at most $\exp(-O(N/T^2))$, the overlap $\braket{0|\gen_k^{\dagger}|\rho_{k,\psi}|\gen_k|0}$ is $O(1/T)$-close to the average (as a result, greater than $1/3T$).
\end{proof}

Now we can replace the projector $\Pi_k$ in~\cref{eq:projectors_attack} with
\begin{align*}
    \widetilde{\Pi_k} = \left(\Big((\widetilde{U_k}^\dagger)_{\mathsf{AB}} \otimes \I_{\mathsf{C}} \Big) (\Pi^{sym}_{\mathsf{AC}} \otimes \I_{\mathsf{B}} )\Big((\widetilde{U_k})_{\mathsf{AB}} \otimes \I_{\mathsf{C}}\Big)\right)^{\otimes \poly},
\end{align*}
where $\widetilde{U_k}$ is the unitary operator corresponding to $\widetilde{\gen}_k$. Then according to~\cref{lem:state-simulation-overlap}, $\ket{\phi_k}^{\otimes \poly} \otimes \ket{\psi}^{\otimes \poly}$ will pass the test with high probability, and $\ket{\phi}^{\otimes \poly} \otimes \ket{\psi}^{\otimes \poly}$ cannot pass the test with high probability, and then plug in the OR lemma~\cref{lem:or-lemma}, we are done. 
\end{comment}


==> oneway_puzzles.tex <==

\section{One-way puzzles from common Haar random states}
In this section, we show how to construct $\owpuzz$ in the CHRS model. The construction is based on two technical lemma: the classical shadow tomography shown in~\cite{HKP20} and the LOCC Haar state indistinguishability shown in~\cite{ananth2024cryptography}.\bnote{Explain the definition of one-way puzzle in the CHRS model, cite AGL24} 

First we need to clarify the definition of one-way puzzle in the CHRS model. The same as the plain model, the puzzle consists of the sampler and the verifier, and the time-efficient/time-inefficient algorithms map into query-efficient/query-inefficient algorithms. 

\begin{definition}[One-way puzzles with query-inefficient verifier in the CHRS model]
    A one-way puzzle with query-inefficient verifier is a pair of sampling and verification algorithms $(\sf{Samp}, \sf{Ver})$ with the following syntax.
    \begin{itemize}
        \item $\sf{Samp}(1^n, \bigotimes_{i=1}^l \ket{\psi_i}^{\otimes l}) \to (k,s)$ is a (not necessarily time-bounded) algorithm that takes $n$ and $l$ copies of $l$ independent random states as input, outputs a pair of classical strings $(k,s)$, where $l=l(n)$ is polynomial in $n$. We refer to $s$ as the puzzle and $k$ as its key.
        \item $\sf{Ver}(k, s, \bigotimes_{i=1}^r \ket{\psi_i}^{\otimes r}) \to \top/\bot$ is a time-unbounded algorithm that on input of any pair classical strings $(k,s)$ halts and outputs $\top/\bot$, where $r=r(n)$ can be arbitrarily function of $n$.
    \end{itemize}
    These satisfy the following properties.
    \begin{itemize}
        \item \textbf{Correctness:} Outputs of the sampler pass verfication with overwhelming probability, i.e.
        \begin{equation*}
            \Pr_{(k,s) \gets \sf{Samp}(1^n, \bigotimes_{i=1}^l \ket{\psi_i}^{\otimes l})} [\sf{Ver}(k,s, \bigotimes_{i=1}^r \ket{\psi_i}^{\otimes r})=\top] = 1 - \negl(n)
        \end{equation*}
        \item \textbf{Security:} Given $s$, for any query-bounded computationally adversary $\calA$
        \begin{equation*}
            \Pr_{(k,s) \gets \sf{Samp}(1^n, \bigotimes_{i=1}^l\ket{\psi_i}^{\otimes l})}[\sf{Ver}(\calA(s, \bigotimes_{i=1}^{t}\ket{\psi_i}^{\otimes t}), \bigotimes_{i=1}^r \ket{\psi_i}^{\otimes r}) = \top] = \negl(n)
        \end{equation*}
        where $t=t(n)$ in polynomial in $n$.
    \end{itemize}
\end{definition}\bnote{Added definition of $\owpuzz$ in the CHRS model and mentioned AGL's work}
Similarly we can define one-way puzzle with query-efficient verifier (we call it $\evowpuzz$ in the CHRS model for convenience). \cite{ananth2024cryptography} proposes the definition of $\evowpuzz$ in the CHRS model. They show that unconditional $\evowpuzz$ in the CHRS model does not exist. In this section, we show that (query-inefficiently verifiable) $\owpuzz$ in the CHRS model exists unconditionally, which is consistent with their results.

The construction of $\owpuzz$ relies heavily on the classical shadow tomography~\cite{HKP20}, so here we first describe how to sample classical shadow tomography and also the theoretical guarantee of shadow tomography. Assume we have $N$ copies of a state $\rho$ and we want to estimate the observables $O_1, \dots, O_M$ with the copies of $\rho$. One can do this by just doing independent random Clifford measurements over all the copies of $\rho$. Namely, we can sample random Clifford unitaries $C_1, \dots, C_N$, and then measure $C_i\rho C_i^\dagger$ and record their measurement results $b_1, \dots, b_N$. We call the collection of $b_i, C_i$ the classical shadow tomography of the state $\rho$, denoted as $\sf{ShadowGen}(\rho, N)$, which can be sampled without prior knowledge of the observables. The theoretical guarantee is shown in the following lemma.
\begin{lemma}[Classical shadow tomography, adapted from~\cite{HKP20}]\label{lem:classical-shadow-tomography}
    For any $n$-qubit observables $O_1, \dots, O_M$, and accuracy parameter $\eps, \delta \in [0,1]$. Let $N \geq \frac{204}{\eps^2}\log(2M/\delta)\max_{1\leq i \leq M}\tr O_i^2$. Then for any $n$-qubit state $\rho$, let $\sf{ShadowGen}(\rho, N)$ be the classical shadow tomography of $N$ copies of $\rho$. Then there is a time-unbounded classical algorithm that can give an estimation $\hat{o}_i$ on all the observables $\tr O_i \rho$ given $\sf{ShadowGen}(\rho, N)$ such that
    \begin{equation*}
        |\hat{o}_i - \tr(O_i \rho)| \leq \eps \, \forall i \in [1,M]
    \end{equation*}
    with probability at least $1-\delta$.
\end{lemma}

%First we describe how to sample the puzzle. Take $\ncopy$ copies of each $l$-qubit CHRS state where $l$ ranges from $n$ to $2n$. Namely, we take $\ket{\psi_n}^{\otimes \ncopy}\otimes \dots \ket{\psi_{2n}}^{\otimes \ncopy}$. Then for all $l \in [n,2n]$, we sample a random bit $k_l$ and ten random $l$-qubit Clifford gates $C_{l,1}, \dots, C_{l,\ncopy}$. Then the sampler makes measurement on computational basis of $C_{l,i}Z^{k_l}\ket{\psi_l}(1 \leq i \leq \ncopy)$, and outputs $\ncopy$ bit strings $b_{l,i} \in \{0,1\}^l$. The sampler will output $k_n\dots k_{2n}$ as the key and all the $C_{l,i}$ and $b_{l,i}$ as the puzzle.

Now we can describe the puzzle. Take $\ncopy$ copies of each $l$-qubit CHRS state where $n \leq l \leq 2n$. For each $l \in [n,2n]$, the sampler chooses a random bit $k_l \in \{0,1\}$ and then generates a classical shadow tomography of $\ncopy$ copies of $(Z^{k_l}_1 \otimes \I )\ket{\psi_l}$. The sampler will output $k_n \dots k_{2n}$ as the key and the collection of $\sf{ShadowGen}((Z^{k_l}_1 \otimes \I)\ket{\psi_l}\bra{\psi_l}(Z^{k_l}\otimes \I))$ as the puzzle.

The verifier of the puzzle relies on~\cref{lem:classical-shadow-tomography}. For any $l \in [n, 2n]$, the verifier takes as input $k_l$ and $\sf{ShadowGen}((Z^{k_l}_1\otimes \I)\ket{\psi_l}\bra{\psi_l}(Z^{k_l}_1 \otimes \I))$. The verifier estimates the observable $(Z^{k_l}_1 \otimes \I)\ket{\psi_l}\bra{\psi_l}(Z^{k_l}_1 \otimes \I)$ according to the classical shadow tomography. The verifier accepts if for at least 3/4 fraction of $l$, the estimation of the corresponding observable is greater than 1/2. The estimation of $(Z^{k_l}_1 \otimes \I)\ket{\psi_l}\bra{\psi_l}(Z^{k_l}_1 \otimes \I)$ needs the classical description of $\ket{\psi_l}$, which can be done if the verifier has access to exponentially many copies of $\ket{\psi_l}$.

% Now we can describe how to verify the puzzle. For any $l \in [n,2n]$, we know $(C_{l_i}, b_{l_i})$ is a classical shadow of $Z^{k_l}\ket{\psi_l}$. The shadow tomography algorithm then just takes the classical shadow as the input and measures $O_{l,0} = \ket{\psi_l}\bra{\psi_l}$ and $O_{l,1} = Z\ket{\psi_l}\bra{\psi_l}Z$. The verifier accepts only if the estimation of $O_{l,k_l}$ is greater than 1/2 for all at least $3/4$ different $l$'s.

According to~\cref{lem:classical-shadow-tomography}, set $\eps = 1/3$ and $\delta = 1/10$, the probability that the estimation of $Z_1^{k_l} \otimes \I$ deviates by at least $1/2$ is less than 1/10 when the number of copies of the classical shadow $N \geq 204 \cdot 9 \cdot \log (2 \cdot 100)$, for which $\ncopy$ copy is enough. Since $Z^{k_l}\ket{\psi_l}$ measures 1 on $Z^{k_l}\ket{\psi_l}\bra{\psi_l}Z^{k_l}$, the probability that the estimation is lower than 1/2 is at most 1/10. 

Thus by a Chernoff bound, the probability that a puzzle is not accepted by the verifier is exponentially small, so the correctness of the puzzle follows.

As for the security, first we show that for any adversary $\calA$ that does not have access to the common Haar random states, $\calA$ can find a key that passes the test with only exponentially small probability. This is because $\ket{\psi_l}$ and $Z\ket{\psi_l}$ are essentially symmetric if the adversary has no information about $\ket{\psi}$, so the best he can do is to guess the key randomly. Therefore the adversary can guess each $k_l$ correctly with probability at most 1/2, and if the adversary does not guess the correct key, the probability that the estimation of $Z^{k_l}\ket{\psi_l}\bra{\psi_l}Z^{k_l}$ is greater than 1/2 is at most 1/10 according to~\cref{lem:classical-shadow-tomography} and $|\braket{\psi_l|Z|\psi_l}|^2$ does not exceed 1/10 except for exponentially small probability. Then by Chernoff bound, the adversary can pass the verification with only exponentially small probability.

What if the adversary can access polynomially many copies of the common Haar random states? Notice that the whole process can be viewed as  This does not help very much by the following lemma.

\begin{lemma}[LOCC Haar indistinguishability, adapted from~\cite{ananth2024cryptography}]\label{lem:locc-harr-indi}
    For positive integers $s, t, n_1, \dots, n_s$, define
    \begin{align*}
        \rho_{\sfA\sfB} &\coloneqq \bigotimes_{i=1}^s \E_{\ket{\psi_i} \gets \calH_{n_i}} \left[ (\ket{\psi_i}\bra{\psi_i}^{\otimes t})_{\sfA_i} \otimes (\ket{\psi_i}\bra{\psi_i}^{\otimes t})_{\sfB_i} \right] \\
        \sigma_{\sfA\sfB} &\coloneqq \bigotimes_{i=1}^s \E_{\ket{\psi_i} \gets \calH_{n_i}} \left[ (\ket{\psi_i}\bra{\psi_i}^{\otimes t})_{\sfA_i} \right] \otimes \bigotimes_{i=1}^s \E_{\ket{\phi_i} \gets \calH_{n_i}} \left[ (\ket{\phi_i}\bra{\phi_i}^{\otimes t})_{\sfB_i} \right],
    \end{align*}
    where $\sfA = (\sfA_1, \dots, \sfA_s)$, $\sfB = (\sfB_1, \dots, \sfB_s)$. Then $\rho_{\sfA\sfB}$ and $\sigma_{\sfA\sfB}$ are $O(\sum_{i=1}^s t^2/2^{n_i})$-LOCC indistinguishable.
\end{lemma}
Notice that the one-way puzzle can be viewed as an LOCC-protocol between the sampler and the adversary, thus according to~\cref{lem:locc-harr-indi}, the oracle can be replaced by an oracle that is sampled from fresh Haar random states up to an exponentially small factor, which does not provide any information about the common Haar random state. Thus by a hybrid argument, any adversary with access to polynomially many copies of the common Haar random states can only guess half of the key. We formalize this idea in the following lemma.

\begin{theorem}\label{thm:owpuzz-security}
    For any adversary $\calA^{\{\ket{\psi_l}\}}$ with access to polynomially many copies of the CHRS states, if the sampler samples a puzzle $(k, s)$ and inputs the puzzle $s$ to $\calA^{\{\ket{\psi_l}\}}$, then , $\calA$ can guess at most 3/5 fraction of all the keys except for exponentially small probability.
\end{theorem}
\begin{proof}
    Consider the adversary $\calA^{\{\ket{\psi'_l}\}}$. The algorithm is exactly the same algorithm as $\calA^{\ket{\psi_l}}$ but the $\ket{\psi_l'}$ are independently sampled Haar random states. Then essentially the adversary gains no information about $k$. For any $l$, if we replace $k$ with $k \oplus 1$ and replace $\ket{\psi_l}$ with $(Z_1 \otimes \I)\ket{\psi_l}$, then the distribution of the shadow tomography is exactly is the same, while the key is flipped. Thus the probability that $\calA^{\ket{\psi_l'}}$ can guess the correct $k_l$ does not exceed 1/2.

    So what's the case for the real-world adversary $\calA^{\{\ket{\psi_l}\}}$? We can construct the following non-local game.
    \begin{itemize}
        \item Alice runs the algorithm $\sf{Samp}^{\{\ket{\psi_l}\}}(1^n)$ samples a pair of puzzle $(k, s)$ and sends $s$ to Bob.
        \item Bob runs $\calA^{\{\ket{\psi_l}\}}(s)$ and outputs a key $k'$. Bob then sends $k'$ back to Alice.
        \item Alice compares $k$ and $k'$. If 3/5 fraction of all the bits agree, then Alice accepts. Otherwise Alice rejects.
    \end{itemize}
    This is an LOCC protocol and the acceptance probability is exactly the probability that $\calA$ can guess at least 3/5 of all the keys. According to~\cref{lem:locc-harr-indi}, we can replace the CHRS oracle on Bob's side with freshly sampled random states, with only a $O(t^2n/2^n)$ overhead. If we replace the CHRS oracle, we get the following idealized game,
    \begin{itemize}
        \item Alice runs the algorithm $\sf{Samp}^{\{\ket{\psi_l}\}}(1^n)$ samples a pair of puzzle $(k, s)$ and sends $s$ to Bob.
        \item Bob runs $\calA^{\{\ket{\psi_l'}\}}(s)$ and outputs a key $k'$. Bob then sends $k'$ back to Alice.
        \item Alice compares $k$ and $k'$. If 3/5 fraction of all the bits agree, then Alice accepts. Otherwise Alice rejects.
    \end{itemize}
    For the idealized game, as we have analyzed before, the adversary can guess each $k_l$ with probability only 1/2, so according to the Chernoff bound, Alice accepts only with exponentially small probability. So in the original game, Alice also accepts with exponentially small probability.
\end{proof}

\begin{corollary}
    For any adversary $\calA^{\{\ket{\psi_l}\}}$ with access to polynomially many copies of the CHRS states, $\calA^{\ket{\psi_l}}$ takes a puzzle $s$ as input and output a key $k'$. $k'$ can pass the verification with only exponentially small probability.
\end{corollary}
\begin{proof}
    According to~\cref{thm:owpuzz-security}, $k'$ coincides with at most 3/5 fractions of the bit strings. For any $l$ that $k_l' \neq k_l$, then since $\braket{\psi_l| Z_1^{k_l} \otimes \I |\psi_l}$ is negligible except for exponentially small probability, 
    \begin{equation*}
        \tr Z^{k_l'}\ket{\psi_l}\bra{\psi_l}Z^{k_l'}Z^{k_l}\ket{\psi_l}\bra{\psi_l} Z^{k_l} 
    \end{equation*} 
     is negligible with high probability. Since we take $\ncopy$ copies of classical shadow tomography, the estimation of the observable deviates from the expectation at most 1/3 with probability at least 9/10, so each wrong key will pass the test (estimation greater than 1/2) with probability at most 1/10, but $1/10+3/5 \leq 3/4$, so according to the Chernoff bound, the acceptance probability is expoentially small.
\end{proof}
